Multi-fairness under class-imbalance

Recent studies showed that datasets used in fairness-aware machine learning for multiple protected attributes (referred to as multi-discrimination hereafter) are often imbalanced. The class-imbalance problem is more severe for the often underrepresented protected group (e.g. female, non-white, etc.) in the critical minority class. Still, existing methods focus only on the overall error-discrimination trade-off, ignoring the imbalance problem, thus amplifying the prevalent bias in the minority classes. Therefore, solutions are needed to solve the combined problem of multi-discrimination and class-imbalance. To this end, we introduce a new fairness measure, Multi-Max Mistreatment (MMM), which considers both (multi-attribute) protected group and class membership of instances to measure discrimination. To solve the combined problem, we propose a boosting approach that incorporates MMM-costs in the distribution update and post-training selects the optimal trade-off among accurate, balanced, and fair solutions. The experimental results show the superiority of our approach against state-of-the-art methods in producing the best balanced performance across groups and classes and the best accuracy for the protected groups in the minority class.

==> theory.tex <==

We derive the effectiveness of our boosting algorithm in producing \eqDM-fair outcomes. We assume that the boosting based part of training the partial ensembles of our algorithm will converge w.r.t. the classification loss ($O_1$) when trained for a sufficient number of weak learners; the proof for this assumption can be based on the convergence proof of vanilla AdaBoost~\cite{mukherjee2013convergence_adaboost}.
%\color{black}
%\vspace{-1mm}
\begin{lemma}\label{lem}
As classification (0-1) loss ($O_1$) of a partial ensemble $H_{t'}=\sum_{l=1}^{t'}\alpha_{l}h_{l}$ trained for a protected attribute $S_j$ via the in-processing of \Multifair~Algorithm (Eq. \ref{eq:weight_update}) 
converges, cumulative fairness cost $\delta f_{j}^{t'}\in\{|\delta {FPR}_j^{1:t'}|,|\delta {FNR}_j^{1:t'}|\}$ (Eq. \ref{fcm}) of each partial ensemble w.r.t $S_j$ also tends to converge to a low value. 
\small
\begin{equation*}
    \begin{aligned}
     P_{t'}(\hat{y_i} \ne y_i) - P_{t}(\hat{y_i} \ne y_i) \rightarrow 0;t'>t
     \implies \delta f_{j}^{t'} \rightarrow \mu;\forall{H_{t'}},~as~t'\uparrow\phantom{1};\phantom{123231313}\\
     \normalsize\text{where }\small~\delta f_{j}^{t'}\in\{|\delta {FPR}_j^{1:t'}|,|\delta {FNR}_j^{1:t'}|\};~\mu~\normalsize\text{is a tolerable discrimination for}\small~S_j\text{ in any class}
    \end{aligned}
\end{equation*}
\normalsize

\end{lemma}
\noindent Lemma \ref{lem} guarantees that if the assumption of convergence on $O_1$ holds, then the \Multifair~algorithm trained for any protected attribute $S_j$ will always converge to a very low $\eqDM_S$ loss ($O_3$). 
\begin{theorem}\label{theo1}
A final ensemble $H_{t^*}$ given as output by the \Multifair~algorithm trained w.r.t a set of $k$ protected attributes $S=\{S_1,...,S_k\}$, with any choice of $ \vec{U}$, upon being chosen from a set of partial ensembles converged w.r.t $O_1$ and $O_3$, will be a \eqDM-fair classifier with a threshold $(\mu+\epsilon)$.

\small
\begin{equation*}
    \eqDM_{S} \le (\mu+\epsilon);~S=\{S_1,...,S_k\}
    %CDM_j\le 2(\Delta + \epsilon);~ \forall{S_j}\in S
\end{equation*}
\normalsize
where $\epsilon$ is trade-off for $O_3$  w.r.t $O_1$ and $O_2$. 
%(proof given in Appendix E).
%\vspace{+2mm}
\end{theorem}
%\vspace{-2mm}
\normalsize
\noindent Lemma~\ref{lem} and Theorem~\ref{theo1} together characterize the conditions by which in-training  \Multifair~algorithm upon being trained for sufficiently large number of weak learners, will converge in \mf~with fair outcomes \small$DM_j\le 2\mu $, where \small$\mu$\normalsize~is a tolerable discrimination in any class \small$\forall{S_j}\in S$\normalsize.
\begin{proof}
From Lemma~\ref{lem} we get to know that the in-training part of \Multifair~algorithm trained w.r.t protected attribute $S_j$, upon classification loss convergence will give a set of fair partial ensembles $\{H_t|\delta f_{j}^{t} \approx \mu\}$ w.r.t $S_j\in S$. Now, let $S_j\in S$ be a protected attribute that dominates $fc_t(x_i)$ (Eq. \ref{s_phi}), i.e:
% \begin{equation}
%     \begin{aligned}
%         \max ()
%     \end{aligned}
% \end{equation}
% %groups defined by $S_j$ is discriminated the most among all the groups defined $S$ from $H_t$. 
% This implies, 
\small
\begin{equation}\label{eq:theo1_1}
    \delta f_{j}^t\ge \delta f_{k}^t, \forall{S_k}\in S
\end{equation}
\normalsize
%$\delta f_{j}^t\ge \delta f_{k}^t, \forall{S_k}\in S$.
From Def.~\ref{def: DB}, and Eq.~%\ref{eq: eqdm}, \ref{eq:l2_6} and 
\ref{eq:theo1_1} we get that,
\small
\begin{equation}\label{eq:theo1_2}
    CDM_k\le 2\delta f_{j}^t;~ \forall{S_k}\in S
\end{equation}
\normalsize
%$CDM_k\le 2\delta f_{j}^t;~ \forall{S_k}\in S$. 
Now, following Lemma \ref{lem} we get that as $H_t$ approaches convergence, $\delta f_{j}^t \rightarrow \mu$, where $\mu$ is a small value ($\approx 0$). Again, from Eqs.~\ref{eq:l2_6}, and~\ref{eq:theo1_2} we get,
\begin{equation}\label{eq:theo1_3}
\begin{aligned}
    \eqDM_S\leq \mu 
\end{aligned}
\end{equation}
Assuming $o_3^{min}=\mu$, where $o_3^{min}$ is the best available solution value for $O_3$ after convergence of $H_t$. Using the post-training selection steps (\underline{$Step_1-Step_4$}) with any $\vec{U}$, we get $H_{t^*}$, which gives a solution vector $[o_1,o_2,o_3]_f \in \mathbb{PF}$. Assuming the given condition of $H_{t^*}$ being chosen from the set of the partial ensemble converged in $O1$ and $O3$, we get that worst possible value for $o_3= o_3^{min}+\epsilon$, where $\epsilon$ is small divergence from the optima $o_3^*$. This implies that for predictions by $H_{t^*}$,
\begin{equation}
  MMM_S \le (\mu+\epsilon)   
\end{equation}
%$MMM_S \le (\Delta+\epsilon);~ \forall{S_j}\in S$.
$\blacksquare$
\end{proof}
